Scalable and Secure Aggregation in Distributed Networks

We consider the problem of computing an aggregation function in a \emph{secure} and \emph{scalable} way. Whereas previous distributed solutions with similar security guarantees have a communication cost of $O(n^3)$, we present a distributed protocol that requires only a communication complexity of $O(n\log^3 n)$, which we prove is near-optimal. Our protocol ensures perfect security against a computationally-bounded adversary, tolerates $(1/2-\epsilon)n$ malicious nodes for any constant $1/2 > \epsilon > 0$ (not depending on $n$), and outputs the exact value of the aggregated function with high probability.

==> layout.tex <==
In this section, we describe the first phase of the algorithm whose purpose is to construct a structured layout. The layout we want to achieve is a partition of the nodes into clusters $C_1, \ldots, C_g$ of size $O(\log n)$. The clusters will be organized in a ring such that each node is connected to all the other nodes in its cluster as well as to all the nodes of the previous and the next cluster. This means that each individual node is connected to $O(\log n)$ nodes in this structured layout. Moreover, we require that in each cluster there is a majority of honest nodes. The construction of a layout achieving such a property is a necessary precondition to ensure the security property of our protocol. In this sense, the construction of the layout can be done offline as a preprocessing step before the execution of the protocol. Recall that the number of malicious nodes $\tau$ controlled by the adversary is strictly upper bounded by $(1/2-\epsilon)n$ for some constant $\epsilon>0$ independent of $n$. 

The strategy used to construct this layout has to be carefully designed such that whatever are the actions of the malicious nodes, we have the guarantee that they will not gain the majority in any cluster (except with small probability). To realize this, we use a technique described in \cite{Baumgart2007}, which consists in using a hash of the public key of a node to generate a random number. To do that we assume that the hash function that will be used is public (it can be for instance given by the CA along with the public key when the node registers) and for practical purpose it is sufficient that the hash function returns a value between $\{1, \ldots, n^3\}$ to avoid the risk of collision between the hashes of two different nodes.  

We assume that there exists a cluster of $O(\log n)$ nodes such that at least half of them are honest. When the CA registers a node, it also indicates to it the identities of these nodes 
The nodes of this cluster can compute locally the random ordering $x_1,...,x_n$ that is induced by the hash of the public keys. This random ordering will be used to define the clusters: given a constant\footnote{$k$ is a parameter of the protocol and therefore fixed in advance. For instance, in our experiments we used $k=?????$.} $k$, for $1\leq i \leq n/(k\log n)$, we set $C_i=\{x_{(i-1)k\log n+1}, \ldots x_{ik\log n}\}$. Theorem \ref{thm:partition} that in this setting, there will be a majority of honest nodes in each cluster with high probability.

\begin{theorem}\label{thm:partition}
Given a random partition of $n$ nodes, with at most $(1/2-\epsilon)n$ malicious nodes for some constant $\epsilon > 0$, in $n/k\log(n)$ sets each of size $k\log(n)$,  with high probability in $n$, there is a majority of honest nodes in each set (provided $k$ is large enough).
\end{theorem}

\begin{proof}
See the Appendix for the proof. \qed
\end{proof}
